Effects of Hoyle state de-excitation on $\nu p$-process nucleosynthesis and Galactic chemical evolution

The partcle-induced hadronic de-excitation of the Hoyle state in $^{12}$C induced by inelastic scattering in a hot and dense plasma can enhance the triple-alpha reaction rate. This prevents the production of heavy nuclei within the neutrino-driven winds of core-collapse supernovae and raises a question as to the contribution of proton-rich neutrino-driven winds as the origin of $p$-nuclei in the solar system abundances. Here we study $\nu p$-process nucleosynthesis in proton-rich neutrino-driven winds relevant to the production of $^{92,94}\mathrm{Mo}$ and $^{96,98}\mathrm{Ru}$ by considering such particle-induced de-excitation. We show that the enhancement of the triple-alpha reaction rate induced by neutron inelastic scattering hardly affects the $\nu p$-process, while the proton scattering contributes to the nucleosynthesis in proton-rich neutrino-driven winds at low temperature. The associated enhanced triple-alpha reaction rate decreases the production of $^{92,94}\mathrm{Mo}$ and $^{96,98}\mathrm{Ru}$ in a wind model of ordinary core-collapse supernovae. On the other hand, the abundances of these $p$-nuclei increase in an energetic hypernova wind model. Hence, we calculate the galactic chemical evolution of $^{92,94}\mathrm{Mo}$ and $^{96,98}\mathrm{Ru}$ by taking account of both contributions from core-collapse supernovae and hypernovae. We show that the hypernova $\nu p$-process can enhance the calculated solar isotopic fractions of $^{92,94}\mathrm{Mo}$ and $^{96,98}\mathrm{Ru}$ and make a significant impact on the GCE of $p$-nuclei regardless of the particle-induced Hoyle state de-excitation.

==> ref_MK1.tex <==
\begin{thebibliography}{999}
\bibitem[Arnould(1976)]{1976A&A....46..117A} Arnould, M.\ 1976, \aap, 46, 117
   
\bibitem[Arnould \& Goriely(2006)]{arn06} Arnould, M., \& Goriely, S.\ 2006, Nuclear Physics A, 777, 157 

\bibitem[Arnould \& Goriely(2003)]{arn03} Arnould, M., \& Goriely, S.\ 2003, \physrep, 384, 1 

\bibitem[Audouze(1970)]{1970A&A.....8..436A} Audouze, J.\ 1970, \aap, 8, 436 

\bibitem[Burbidge et al.(1957)]{1957RvMP...29..547B} Burbidge, E.~M., Burbidge, G.~R., Fowler, W.~A., \& Hoyle, F.\ 1957, Reviews of Modern Physics, 29, 547 

\bibitem[Costa et al.(2000)]{cos00} Costa, V., Rayet, M., Zappal{\`a}, R.~A., \& Arnould, M.\ 2000, \aap, 358, L67
https://www.overleaf.com/project/5fa2b3d6a0af180b51241f60  
\bibitem[Frank-Kamenetskii(1961)]{1961SvA.....5...66F} Frank-Kamenetskii, D.~A.\ 1961, \sovast, 5, 66 

\bibitem[Fr{\"o}hlich et al.(2006a)]{fro06a} Fr{\"o}hlich, C., et al.\ 2006a, \apj, 637, 415 

\bibitem[Fr{\"o}hlich et al.(2006b)]{fro06b} Fr{\"o}hlich, C., Mart{\'{\i}}nez-Pinedo, G., Liebend{\"o}rfer, M., Thielemann, F.-K., Bravo, E., Hix, W.~R., Langanke, K., \& Zinner, N.~T.\ 2006b, Physical Review Letters, 96, 142502 

\bibitem[Goriely et al.(2001)]{2001A&A...375L..35G} Goriely, S., Arnould, M., Borzov, I., \& Rayet, M.\ 2001, \aap, 375, L35
  
  
\bibitem[Goriely et al.(2005)]{gor05} Goriely, S., Garc{\'{\i}}a-Senz, D., Bravo, E., \& Jos{\'e}, J.\ 2005, \aap, 444, L1 

\bibitem[Goriely et al.(2002)]{gor02} Goriely, S., Jos\'e, J., Hernanz, M., Rayet, M., \& Arnould, M.  2002, \aap, 383, L27

bibitem[Hainebach et al.(1976)]{1976ApJ...205..920H} Hainebach, K.~L., Schramm, D.~N., \& Blake, J.~B.\ 1976, \apj, 205, 920 

\bibitem[Hayakawa et al.(2008)]{hay08} Hayakawa, T., Iwamoto, N., Kajino, T., Shizuma, T., Umeda, H., \& Nomoto, K.\ 2008, \apj, 685, 1089 

\bibitem[Hainebach et al.(1976)]{1976ApJ...205..920H} Hainebach, K.~L., Schramm, D.~N., \& Blake, J.~B.\ 1976, \apj, 205, 920
  
\bibitem[Hoffman et al.(1996)]{hof96} Hoffman, R.~D., 
Woosley, S.~E., Fuller, G.~M., \& Meyer, B.~S.\ 1996, \apj, 460, 478 

\bibitem[Howard et al.(1991)Howard, Meyer, \& Woosley]{how91} Howard, W.~M., Meyer, B.~S., \& Woosley, S.~E.\ 1991, \apjl, 373, L5

\bibitem[Howard \& Meyer(1992)]{how92} Howard, W.M., \& Meyer, B.S. 1992, in Nuclei in the Cosmos Symp. 2,
  ed. F. K\"aeppeler, \& K. Wisshak (Bristol; Philadelphia: Institute of Physics Pub.), 575

\bibitem[Ito(1961)]{1961PThPh..26..990I} Ito, K.\ 1961, Progress of Theoretical Physics, 26, 990
  
\bibitem[Iwamoto et al.(2005)Iwamoto, Umeda, \& Nomoto]{iwa05} Iwamoto, N., Umeda, H., \& Nomoto, K.\ 2005, in Origin of Matter and Evolution of Galaxies 2003,
  ed. M. Terasawa et al. (Hackensack: World Scientific), 493
  
\bibitem[Kusakabe et al.(2011)]{2011ApJ...726...25K} Kusakabe, M., Iwamoto, N., \& Nomoto, K.\ 2011, \apj, 726, 25 

\bibitem[Kusakabe \& Mathews(2018)]{2018ApJ...854..183K} Kusakabe, M. \& Mathews, G.~J.\ 2018, \apj, 854, 183. doi:10.3847/1538-4357/aaa125
  
\bibitem[Lambert(1992)]{lam92} Lambert, D.~L.\ 1992, \aapr, 3, 201

\bibitem[Meyer(1994)]{mey94} Meyer, B.~S.\ 1994, \araa, 32, 153 

\bibitem[Hainebach et al.(1976)]{1976ApJ...205..920H} Hainebach, K.~L., Schramm, D.~N., \& Blake, J.~B.\ 1976, \apj, 205, 920

\bibitem[Prantzos et al.(1990)]{pra90} Prantzos, N., Hashimoto, M.,
  Rayet, M., \& Arnould, M.  1990, \aap, 238, 455
    
\bibitem[Pruet et al.(2005)]{pru05} Pruet, J., Woosley, 
  S.~E., Buras, R., Janka, H.-T., \& Hoffman, R.~D.\ 2005, \apj, 623, 325
    
\bibitem[Pruet et al.(2006)]{pru06} Pruet, J., Hoffman, R.~D., Woosley, S.~E., Janka, H.-T., \& Buras, R.\ 2006, \apj, 644, 1028 

\bibitem[Rauscher et al.(2002)]{rau02} Rauscher, T., Heger, A., Hoffman, R.~D., \& Woosley, S.~E.\ 2002, \apj, 576, 323 

\bibitem[Rayet et al.(1990)Rayet, Prantzos, \& Arnould]{ray90} Rayet, M., Prantzos, N., \& Arnould, M.  1990, \aap, 227, 271

\bibitem[Rayet et al.(1995)]{ray95} Rayet, M., Arnould, M., Hashimoto, M., Prantzos, N.,\& Nomoto., K.  1995, \aap, 298, 517

\bibitem[Travaglio et al.(2011)]{2011ApJ...739...93T} Travaglio, C., R{\"o}pke, F.~K., Gallino, R., \& Hillebrandt, W.\ 2011, \apj, 739, 93 
  
\bibitem[Wanajo(2006)]{wan06} Wanajo, S.\ 2006, \apj, 647, 1323
  
\bibitem[Woosley et al.(1990)]{1990ApJ...356..272W} Woosley, S.~E., Hartmann, D.~H., Hoffman, R.~D., \& Haxton, W.~C.\ 1990, \apj, 356, 272
  
\bibitem[Woosley \& Howard(1978)]{woo78} Woosley, S.~E., \& Howard, W.~M.\ 1978, \apjs, 36, 285
  
\bibitem[Bisterzo et al.(2014)]{bist14} Bisterzo, S. et al.,\ 2014, \apj, 787,  10

\bibitem[Ishimaru \& Wanajo(1999)]{ishimaru99} Ishimaru, Y. \& Wanajo, S.\ 1999, \apjl, 511, L33

\bibitem[Wanajo \& Ishimaru(2006)]{wanajo06}  Wanajo, S. \& Ishimaru, Y.\ 2006, Nucl. Phys., A777, 676
    
\end{thebibliography}

